Fixed-Points for Quantitative Equational Logics

We develop a fixed-point extension of quantitative equational logic and give semantics in one-bounded complete quantitative algebras. Unlike previous related work about fixed-points in metric spaces, we are working with the notion of approximate equality rather than exact equality. The result is a novel theory of fixed points which can not only provide solutions to the traditional fixed-point equations but we can also define the rate of convergence to the fixed point. We show that such a theory is the quantitative analogue of a Conway theory and also of an iteration theory; and it reflects the metric coinduction principle. We study the Bellman equation for a Markov decision process as an illustrative example.

==> macros.tex <==
%%%%%%%%%%%%%%%% Macros for this paper  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\qeq}[1]{=_{#1}}
\newcommand{\hb}{\overline{h}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%% Prakash's generic macros  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\newcommand{\singlespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1}\small\CS}
\newcommand{\doublespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.75}\small\CS}
\newcommand{\normalspacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{\BLS}\small\CS}
\makeatother

%       Macros for theorems (thm), propositions (prop), lemmas (lem)
%       corollaries (cor), definitions (defn), conjectures (conj),
%       remark (remark), and examples (example).
%
\theoremstyle{definition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{ax}{Axiom}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{fact}[thm]{Fact}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{axiom}{Axiom} 
%\newtheorem{theorem}[thm]{Theorem}
%\newtheorem{corollary}[thm]{Corollary}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{defin}[thm]{Definition}
\newtheorem{df}[thm]{Definition}
%\newtheorem{definition}[thm]{Definition}
%\newtheorem{example}[thm]{Example}
\newtheorem{claim}[thm]{Claim}
\newtheorem{notn}[thm]{Notation}

\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}

%% Generic and Logic %%
\newcommand{\pair}[2]{\mbox{$\langle #1,\; #2 \rangle$}}
\newcommand{\tuple}[1]{\mbox{$\langle #1 \rangle$}}
\newcommand{\powerset}[1]{\mbox{$\mathcal{P}(#1)$}}
\newcommand{\powfin}[1]{\mbox{$\mathcal{P}_{f}(#1)$}}
\newcommand{\ens}[1]{\mbox{$\{ #1 \}$}}
\newcommand{\alt}{\mathrel{|}}
\newcommand{\ent}{\vdash}
\newcommand{\imp}{\Rightarrow}
%\newcommand{\iff}{\Leftrightarrow}
\newcommand{\deq}{\stackrel{\rm{def}}{=}}
\newcommand{\cont}{\subseteq}
\newcommand{\iso}{\cong}                        % isomorphic ~=
\newcommand{\family}[2]{(#1)_{#2}}              % (X_n)_J or {X_n|J}
\newcommand{\rest}[1]{|_{#1}}                   % restriction S|A
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\interior}[1]{\mathaccent'27#1}
\newcommand{\bor}{\vee}
\newcommand{\band}{\wedge}

%% Lambda calculus
\newcommand{\equiva}{=_{\alpha}}
\newcommand{\redb}{\rightarrow_{\beta}}
\newcommand{\redbs}{\rightarrow_{\beta}^{*}}
\newcommand{\redn}{\rightarrow_n}
\newcommand{\redns}{\rightarrow_c^*}
\newcommand{\FV}[1]{FV(#1)}
\newcommand{\typ}{{Typ}}
\newcommand{\typedlam}{\Lambda_{\sigma}}

%% Linear Logic  %%
\newcommand{\oto}{\mathrel{\relbar\joinrel\circ}}     %Linear hom arrow 
\newcommand{\ofrom}{\mathrel{\relcirc\joinrel\relbar}}   %Lin hom back-arrow 
\newcommand{\x}{\times}
\newcommand{\os}{\oslash}
\newcommand{\oa}{\oplus}
\newcommand{\ox}{\otimes}
\newcommand{\bigox}{\bigotimes}
\newcommand{\bigoa}{\bigoplus}
\newcommand{\tadj}{\dashv}        % in-text adjunction symbol
\newcommand{\girpar}{\bindnasrempa}

%% Category theory %%
\newcommand{\set}{\mbox{$\mathbf{Set}$}}
\newcommand{\rel}{\mbox{$\mathbf{Rel}$}}
\newcommand{\mes}{\mbox{$\mathbf{Mes}$}}
\newcommand{\dom}[1]{\mathsf{dom}(#1)}
\newcommand{\cod}[1]{\mathsf{cod}(#1)}
\renewcommand{\hom}{\mathbf{Hom}}
\newcommand{\nat}{\mathbf{Nat}}
\newcommand{\vect}{\mbox{$\mathbf{Vect}$}}
\newcommand{\cat}{\mbox{$\mathbf{Cat}$}}
\newcommand{\topsp}{\mathbf{Top}}
\newcommand{\ptop}{\mathbf{Top}_{\bullet}}
\newcommand{\abgrp}{\mathbf{AbGrp}}
\newcommand{\mon}{\mathbf{Mon}}
\newcommand{\grp}{\mathbf{Grp}}



%% Analysis %%
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\nif}{\mathb{N}^{\infty}}
\newcommand{\dee}[1]{\mathrm{d}#1}

%% Modal Logic and Semantics %%
\newcommand{\may}[1]{\mbox{$\l #1\r$}}
\newcommand{\must}[1]{\mbox{$[ #1]$}}
\newcommand{\sem}[1]{\mbox{$\llbracket #1 \rrbracket$}}

%% Domain Theory %%
\newcommand{\pre}{\sqsubseteq}
\newcommand{\ua}[1]{\mbox{$\uparrow(#1)$}}    
\newcommand{\da}[1]{\mbox{$\downarrowarrow(#1)$}}    
%\newcommand{\dirsup}{\bigsqcup}
\newcommand{\dirsup}{\mathrel{\setlength{\unitlength}{.7em}\raisebox{-.2em}%
    {\begin{picture}(1,1.5)\put(.5,0){\line(-1,3){.48}}
    \put(.5,0){\vector(1,3){.5}}\end{picture}}}} % directed sup

\newcommand{\lub}{\bigvee}
\newcommand{\glb}{\bigwedge}
\newcommand{\stepfn}[2]{\mbox{$#1\nearrow #2$}}
\newcommand{\dda}{\mathord{\mbox{\makebox[0pt][l]{\raisebox{-.4ex}
                           {$\downarrow$}}$\downarrow$}}}
\newcommand{\dua}{\mathord{\mbox{\makebox[0pt][l]{\raisebox{.4ex}
                           {$\uparrow$}}$\uparrow$}}}

%% Quantum %%
\newcommand{\ket}[1]{\mathop{\big|#1\big>}\nolimits}       % |ket>
\newcommand{\bra}[1]{\mathop{\big<#1\,\big|}\nolimits}     % <bra|
\newcommand{\ketbra}[2]{\mid #1\rangle\!\langle #2 \mid}
\newcommand{\proj}[1]{\mid #1\rangle\!\langle #1 \mid}
\newcommand{\braket}[2]{\langle #1\mid#2\rangle}
\newcommand{\matel}[3]{\langle #1\mid#2\mid#3\rangle}

%% Mac Lane %%
\newcommand{\maclane}{Mac\thinspace Lane}

%% Typesetting proofs

 %      P. TAYLOR'S "END OF PROOF BOX":
 \def\pushright#1{{%            % set up
    \parfillskip=0pt            % so \par doesnt push \square to left
    \widowpenalty=10000         % so we dont break the page before \square
    \displaywidowpenalty=10000  % ditto
    \finalhyphendemerits=0      % TeXbook exercise 14.32
   %                 horizontal
    \leavevmode                 % \nobreak means lines not pages
    \unskip                     % remove previous space or glue
    \nobreak                    % don't break lines
    \hfil                       % ragged right if we spill over
    \penalty50                  % discouragement to do so
    \hskip.2em                  % ensure some space
    \null                       % anchor following \hfill
    \hfill                      % push \square to right
    {#1}                        % the end-of-proof mark (or whatever)
   %                   vertical
    \par}}                      % build paragraph
 % prefer proofs with statements, also space after
 \def\qed{\pushright{\rule{2mm}{3mm}}\penalty-700 \smallskip}

%       Robin's prf environment - modified with PT's  \qed above -
%                               - and with improved pagebreaking - 
%       For laying out a proof:  \begin{proof}{} ... \end{proof}
%       The argument is in case the proof is a continuation as in:
%           \begin{proof}{\ref{four-color} continued} ... \end{proof}
%       if you do not use the argument be careful to use the brackets!

% I have modified this to get rid of the argument.
\renewenvironment{proof}{\begin{trivlist} \item[{\bf ~Proof}.]}%
 {\qed\end{trivlist}}

% M. Barr uses the following:  "It gives a \to that can be used as
% $A\to B$ or $A\to^f B$ or $A\to^{f\o g\o h}B$ or even $A\to^f_gB$.  The
% arrow will grow to fit the label(s).  There are similar definitions for
% \two and \tofro, for which you really might want labels both above and
% below.  Actually, by reading your definition of \kto, I was able to
% simplify this.  But it is still nice to have the optional arguments.
% There is only caveat: although you can have one or the other or both
% labels, if you have both the upper must precede the lower.  These defs
% must either be placed in a style file xor surrounded by \makeatletter
% and \makeatother (but NOT both)."  (Modifications by rags)
% The definitions below look more elaborate than they need to be.
% The reason is that an empty asscript will still cause extra vertical
% spacing and the only way to avoid ugly extra space seems to be using
% some such method as this.

\makeatletter

% In-text size:

\newdimen\w@dth

\def\setw@dth#1#2{\setbox\z@\hbox{\scriptsize $#1$}\w@dth=\wd\z@
\setbox\@ne\hbox{\scriptsize $#2$}\ifnum\w@dth<\wd\@ne \w@dth=\wd\@ne \fi
\advance\w@dth by 1.2em}

\def\t@^#1_#2{\allowbreak\def\n@one{#1}\def\n@two{#2}\mathrel
{\setw@dth{#1}{#2}
\mathop{\hbox to \w@dth{\rightarrowfill}}\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@@^#1{\@ifnextchar_ {\t@^{#1}}{\t@^{#1}_{}}}


\def\t@left^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\hbox to \w@dth{\leftarrowfill}}\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@@left^#1{\@ifnextchar_ {\t@left^{#1}}{\t@left^{#1}_{}}}


\def\two@^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\vcenter{\hbox to \w@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \w@dth{\rightarrowfill}}%
       }\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\tw@@^#1{\@ifnextchar_ {\two@^{#1}}{\two@^{#1}_{}}}


\def\tofr@^#1_#2{\def\n@one{#1}\def\n@two{#2}\mathrel{\setw@dth{#1}{#2}
\mathop{\vcenter{\hbox to \w@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \w@dth{\leftarrowfill}}%
       }\limits
\ifx\n@one\empty\else ^{\box\z@}\fi
\ifx\n@two\empty\else _{\box\@ne}\fi}}
\def\t@fr@^#1{\@ifnextchar_ {\tofr@^{#1}}{\tofr@^{#1}_{}}}

% Displaysize:

\newdimen\W@dth
\def\setW@dth#1#2{\setbox\z@\hbox{$#1$}\W@dth=\wd\z@
\setbox\@ne\hbox{$#2$}\ifnum\W@dth<\wd\@ne \W@dth=\wd\@ne \fi
\advance\W@dth by 1.2em}

\def\T@^#1_#2{\allowbreak\def\N@one{#1}\def\N@two{#2}\mathrel
{\setW@dth{#1}{#2}
\mathop{\hbox to \W@dth{\rightarrowfill}}\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@@^#1{\@ifnextchar_ {\T@^{#1}}{\T@^{#1}_{}}}


\def\T@left^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\hbox to \W@dth{\leftarrowfill}}\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@@left^#1{\@ifnextchar_ {\T@left^{#1}}{\T@left^{#1}_{}}}


\def\Tofr@^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\vcenter{\hbox to \W@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \W@dth{\leftarrowfill}}%
       }\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\T@fr@^#1{\@ifnextchar_ {\Tofr@^{#1}}{\Tofr@^{#1}_{}}}


\def\Two@^#1_#2{\def\N@one{#1}\def\N@two{#2}\mathrel{\setW@dth{#1}{#2}
\mathop{\vcenter{\hbox to \W@dth{\rightarrowfill}\kern-1.7ex
                 \hbox to \W@dth{\rightarrowfill}}%
       }\limits
\ifx\N@one\empty\else ^{\box\z@}\fi
\ifx\N@two\empty\else _{\box\@ne}\fi}}
\def\Tw@@^#1{\@ifnextchar_ {\Two@^{#1}}{\Two@^{#1}_{}}}


\def\to{\@ifnextchar^ {\t@@}{\t@@^{}}}
\def\from{\@ifnextchar^ {\t@@left}{\t@@left^{}}}
\def\two{\@ifnextchar^ {\tw@@}{\tw@@^{}}}
\def\tofro{\@ifnextchar^ {\t@fr@}{\t@fr@^{}}}
\def\To{\@ifnextchar^ {\T@@}{\T@@^{}}}
\def\From{\@ifnextchar^ {\T@@left}{\T@@left^{}}}
\def\Two{\@ifnextchar^ {\Tw@@}{\Tw@@^{}}}
\def\Tofro{\@ifnextchar^ {\T@fr@}{\T@fr@^{}}}

\makeatother


\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}


\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\mfrA}{\mathfrak{A}}
\newcommand{\mfrB}{\mathfrak{B}}
\newcommand{\mfrC}{\mathfrak{C}}
\newcommand{\mfrD}{\mathfrak{D}}
\newcommand{\mfrE}{\mathfrak{E}}
\newcommand{\mfrF}{\mathfrak{F}}
\newcommand{\mfrG}{\mathfrak{G}}
\newcommand{\mfrH}{\mathfrak{H}}
\newcommand{\mfrI}{\mathfrak{I}}
\newcommand{\mfrJ}{\mathfrak{J}}
\newcommand{\mfrK}{\mathfrak{K}}
\newcommand{\mfrL}{\mathfrak{L}}
\newcommand{\mfrM}{\mathfrak{M}}
\newcommand{\mfrN}{\mathfrak{N}}
\newcommand{\mfrO}{\mathfrak{O}}
\newcommand{\mfrP}{\mathfrak{P}}
\newcommand{\mfrQ}{\mathfrak{Q}}
\newcommand{\mfrR}{\mathfrak{R}}
\newcommand{\mfrS}{\mathfrak{S}}
\newcommand{\mfrT}{\mathfrak{T}}
\newcommand{\mfrU}{\mathfrak{U}}
\newcommand{\mfrV}{\mathfrak{V}}
\newcommand{\mfrW}{\mathfrak{W}}
\newcommand{\mfrX}{\mathfrak{X}}
\newcommand{\mfrY}{\mathfrak{Y}}
\newcommand{\mfrZ}{\mathfrak{Z}}

\newcommand{\mfra}{\mathfrak{a}}
\newcommand{\mfrb}{\mathfrak{b}}
\newcommand{\mfrc}{\mathfrak{c}}
\newcommand{\mfrd}{\mathfrak{d}}
\newcommand{\mfre}{\mathfrak{e}}
\newcommand{\mfrf}{\mathfrak{f}}
\newcommand{\mfrg}{\mathfrak{g}}
\newcommand{\mfrh}{\mathfrak{h}}
\newcommand{\mfri}{\mathfrak{i}}
\newcommand{\mfrj}{\mathfrak{j}}
\newcommand{\mfrk}{\mathfrak{k}}
\newcommand{\mfrl}{\mathfrak{l}}
\newcommand{\mfrm}{\mathfrak{m}}
\newcommand{\mfrn}{\mathfrak{n}}
\newcommand{\mfro}{\mathfrak{o}}
\newcommand{\mfrp}{\mathfrak{p}}
\newcommand{\mfrq}{\mathfrak{q}}
\newcommand{\mfrr}{\mathfrak{r}}
\newcommand{\mfrs}{\mathfrak{s}}
\newcommand{\mfrt}{\mathfrak{t}}
\newcommand{\mfru}{\mathfrak{u}}
\newcommand{\mfrv}{\mathfrak{v}}
\newcommand{\mfrw}{\mathfrak{w}}
\newcommand{\mfrx}{\mathfrak{x}}
\newcommand{\mfry}{\mathfrak{y}}
\newcommand{\mfrz}{\mathfrak{z}}





